Validation of credit default probabilities via multiple testing procedures

We apply multiple testing procedures to the validation of estimated default probabilities in credit rating systems. The goal is to identify rating classes for which the probability of default is estimated inaccurately, while still maintaining a predefined level of committing type I errors as measured by the familywise error rate (FWER) and the false discovery rate (FDR). For FWER, we also consider procedures that take possible discreteness of the data resp. test statistics into account. The performance of these methods is illustrated in a simulation setting and for empirical default data.

==> BsplMTP.tex <==
% latex.default(round(my.summary, 4), file = file.name.latex) 
%
\begin{table}[hbp]
 \begin{center}
 {\footnotesize
 \begin{tabular}{lrrrrrrrrrr}\hline\hline
%\multicolumn{1}{l}{round}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}&
%\multicolumn{1}{c}{}
class $j$ & 1&2 &3 & 4&5 & 6& 7&8 &9 & 11\\

$\widehat{n}_j$ &$43$&$46$&$39$&$39$&$43$&$32$&$26$&$14$&$16$&$2$\\
$p_j$ &$ 0.0001$&$ 0.0003$&$ 0.0006$&$ 0.0011$&$ 0.0020$&$ 0.0035$&$ 0.0060$&$ 0.0105$&$ 0.0185$&$0.0570$\\
defaults &$ 0$&$ 1$&$ 0$&$ 1$&$ 0$&$ 1$&$ 1$&$ 2$&$ 1$&$1$\\
$p$ values&$ 1.0000$&$ 0.0137$&$ 1.0000$&$ 0.0420$&$ 1.0000$&$ 0.1061$&$ 0.1448$&$ 0.0092$&$ 0.2583$&$0.1108$\\\hline
(Bonf)&$ 1.0000$&$ 0.1371$&$ 1.0000$&$ 0.4202$&$ 1.0000$&$ 1.0000$&$ 1.0000$&$ 0.0923$&$ 1.0000$&$1.0000$\\
(Hol)&$1.0000$&$ 0.1234$&$ 1.0000$&$ 0.3361$&$ 1.0000$&$ 0.7429$&$ 0.7429$&$ 0.0923$&$ 1.0000$&$0.7429$\\
(Hom)&$ 1.0000$&$ 0.1234$&$ 1.0000$&$ 0.2941$&$ 1.0000$&$ 0.5307$&$ 0.6457$&$ 0.0830$&$ 1.0000$&$0.5538$\\\hline
(BH)&$ 1.0000$&$ 0.0685$&$ 1.0000$&$ 0.1401$&$ 1.0000$&$ 0.2215$&$ 0.2414$&$ 0.0685$&$ 0.3690$&$0.2215$\\\hline
(d-Bonf)&$1.0000$&$ 0.0580$&$1.0000$&$ 0.1577$&$1.0000$&$ 0.3463$&$ 0.7393$&$ \textbf{0.0336}$&$ 0.9975$&$0.4571$\\
(sd-d-Bonf)&$ 1.0000$&$ \textbf{0.0483}$&$ 1.0000$&$ 0.1343$&$ 1.0000$&$ 0.2800$&$ 0.3096$&$ \textbf{0.0336}$&$ 0.4118$&$0.2800$\\
\hline
\end{tabular}
}
\caption{Adjusted $p$ values for a single realization of defaults with $N=300$ and upgrade-downgrade alternative with $s=-3$ (significant findings in boldface)}
\end{center}
\label{tab:NumExampMTP}
\end{table}
%\begin{sidewaystable}[!tbp]
% \begin{center}
% \begin{tabular}{lrrrrrrrrrr}\hline\hline
%%\multicolumn{1}{l}{round}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}&
%%\multicolumn{1}{c}{}
%class $j$ & 1&2 &3 & 4&5 & 6& 7&8 &9 & 11\\
%
%$\widehat{n}_j$ &$43$&$46$&$39$&$39$&$43$&$32$&$26$&$14$&$16$&$2$\\
%$p_j$ &$ 0.0001$&$ 0.0003$&$ 0.0006$&$ 0.0011$&$ 0.0020$&$ 0.0035$&$ 0.0060$&$ 0.0105$&$ 0.0185$&$0.0570$\\
%observed defaults &$ 0$&$ 1$&$ 0$&$ 1$&$ 0$&$ 1$&$ 1$&$ 2$&$ 1$&$1$\\
%raw $p$ values&$ 1.0000$&$ 0.0137$&$ 1.0000$&$ 0.0420$&$ 1.0000$&$ 0.1061$&$ 0.1448$&$ 0.0092$&$ 0.2583$&$0.1108$\\
%Bonferroni&$ 1.0000$&$ 0.1371$&$ 1.0000$&$ 0.4202$&$ 1.0000$&$ 1.0000$&$ 1.0000$&$ 0.0923$&$ 1.0000$&$1.0000$\\
%Holm&$1.0000$&$ 0.1234$&$ 1.0000$&$ 0.3361$&$ 1.0000$&$ 0.7429$&$ 0.7429$&$ 0.0923$&$ 1.0000$&$0.7429$\\
%Benjamini-Hochberg&$ 1.0000$&$ 0.0685$&$ 1.0000$&$ 0.1401$&$ 1.0000$&$ 0.2215$&$ 0.2414$&$ 0.0685$&$ 0.3690$&$0.2215$\\
%discrete Bonferroni&$1.0000$&$ 0.0580$&$1.0000$&$ 0.1577$&$1.0000$&$ 0.3463$&$ 0.7393$&$ \textbf{0.0336}$&$ 0.9975$&$0.4571$\\
%step-down discrete Bonferroni&$ 1.0000$&$ \textbf{0.0483}$&$ 1.0000$&$ 0.1343$&$ 1.0000$&$ 0.2800$&$ 0.3096$&$ \textbf{0.0336}$&$ 0.4118$&$0.2800$\\
%\hline
%\end{tabular}
%\caption{Adjusted $p$ values for a single realization of defaults with $N=300$ and upgrade-downgrade alternative with $s=-3$ (significant findings in boldface)}
%
%\end{center}
%
%\end{sidewaystable}
%


==> ExampPF.tex <==
\section{Example portfolio and confusion (misclassification) matrices} \label{sec:ExampPFMisClass}
In this section we describe a simple prototype credit portfolio and two types of misclassification matrices. These components will be used in a simulation study in section(s) ... to assess the performance of multiple testing procedures for testing the validity of the r.s.
\subsection{The rating system}
We consider a rating system consisting of $K=14 $ classes. We assume that borrowers are assigned to one of these classes by some model or mechanism (for details see ...). The rating system consists of the following components:
\begin{itemize}
	\item Typical (average) probabilities of default $(PD_1,\ldots,PD_{14})=()$ corresponding to the rating classes $1,\ldots,14$.
	\item Cutpoints $(c_1,\ldots,c_{13})=(...)$ with $PD_1 < c_1 < PD_2 < \cdots < c_{13} < PD_{14}$ that determine for a given default probability of a borrower the rating class she belongs to. This means if a borrower's default probability is estimated to be in the interval $[c_{i-1},c_i)$ she is classified to rating class $i$ (we set $c_0:=0$ and $c_{14}:=1$).
	\item A given probability distribution of borrowers to rating classes, which is depicted in figure \ref{fig:PortfolioGraph} (the exact probabilities are given in the appendix?) 
\end{itemize}
%\begin{figure}[h]
%	\centering
%		%\includegraphics[width=1.00\textwidth]{DistrTMIN.pdf}
%		\includegraphics[height=0.33\textheight]{PortfolioGraph.pdf}
%	\caption{Distribution of rating classes for example portfolio (PDs are given below class numbers)}
%	\label{fig:PortfolioGraph}
%\end{figure} 
These three components make up an artificial example but nevertheless contain some typical (stylized?) features, e.g.
\begin{itemize}
	\item Sparsity of data: most of the default probabilities are rather small, posing statistical challenges when hypotheses tests are performed (besser: resulting in low power for the corresponding binomial hypotheses tests).
	\item depending on the number of borrowers the number $K=14$ of classes may seem large but it is not uncommon to have (?) rs with as much as $K=25$ classes.
\end{itemize}
\footnote{Sollte dieser Satz eher im Simulationsteil stehen?}In the simulation studies in ... we will consider portfolio sizes of $N_{PF}=100, \ldots,1000$. We use fixed (?) simulation from the distribution of borrowers to rating classes, i.e. we ignore the sampling variability that arises from drawing finite sample sizes of borrowers from the distribution. In this sense we describe a conditional settin (?)
\subsection{Two types of misclassification schemes}
We introduce two types of models for the misclassification matrix $\widehat{N}$ (cf. section ...).
\subsubsection{A simple upgrade-downgrade model}
The upgrade-downgrade model $\widehat{N}^1=\widehat{N}^1(s)$ is parametrized by a shift parameter $s \in \{-K,-K+1, \ldots, K-1,K \}$. Each borrower is upgraded by $s$, i.e. if $g$ is the true rating grade of a borrower he/she will be classified to group
\begin{align}
\widehat{g} &=
\begin{cases}
1 & \qquad \text{if $g-s \le 0$,}\\
g-s & \qquad \text{if $g-s \in \{1\ldots,K \}$,}\\
K & \qquad \text{if $g-s \ge K+1$.}
\end{cases}
\end{align}
This model respresents a systematic, monotone error in the rating system (cf. \cite{Rauhmeier06}).
If $s>0$ each borrower is rated too pessimistically (low rating classes corresponding to low default probabilities) resp. for $s<0$ too optimistically. For $s=0$ the ideal classification is obtained. The matrix below gives an example for $N_{PF}=300$, $K=14$ and $s=-3$. 
\setcounter{MaxMatrixCols}{20}
\begin{align}
\widehat{N}^1(-3) &=
\begin{pmatrix}
$ 2$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 5$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$14$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$22$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$46$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$39$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$39$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$43$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$32$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$26$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$14$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$16$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$0$&$0$&$0$&$0$\\
$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$ 0$&$0$&$2$&$0$&$0$&$0$\\
\end{pmatrix}
\label{eq:BsplUpDownMatrix}
\end{align}
In this case the 5, 14 and 22 borrowers from rating classes 2, 3 and 4 are upgraded to rating class 1, 46 borrowers from grade 5 are assigned to class 2 etc.\\
Even though $s$ is a metric variable it may be more appropriate to interpret its influence on $\widehat{N}^1$ in an ordinal way, i.e. $\widehat{N}^1(2)$ is more pessimistic than $\widehat{N}^1(1)$ but not "twice" as pessimistic.
\subsubsection{An upgrade-downgrade model based on logistic regression}
The model $\widehat{N}^1=\widehat{N}^1(\beta)$ is parametrized by a parameter $\beta$ which determines whether resp. how strongly each borrower is classified too optimistically ($\beta<1$), too pessimistically ($\beta >1$) or perfectly ($\beta=1$). Table ... gives an example for $N_{PF}=100$ and $\beta=...$. The interpretation of $\beta$ is intended to be more qualitative than quantitative. Even though $\beta$ is a metric variable it may be more appropriate to interpret its influence on $\widehat{N}^1$ in an ordinal way, i.e. $\widehat{N}^1(2)$ is more pessimistic than $\widehat{N}^1(1)$ but not "twice" as pessimistic.

As an easy way of obtaining suitable matrices $\widehat{N}^1(\beta)$ we use the following approach.\footnote{We do not propose this model as a realistic model for the default probabilities, indeed we are not concerned with model selection at all. For our purposes only the matrix $\widehat{N}^1(\beta)$ is relevant, irrespectively from the specific way it is constructed. In this sense the viewpoint taken is nonparametric. However, if a specific model $P(Y=1|X=x)=f(x,\theta)$ is used it may make sense to investigate the corresponding misclassification matrices resulting from e.g. estimation uncertainty of the parameter $\theta$.} Assume that the true default probability for $x \in \reell$ is described by $P(Y=1|X=x)=\exp(x)/(1+\exp(x))$, i.e. assume a univariate logistic regression model with true regression parameter $\beta_1=1$ and without intercept term. Then we have (with a slight abuse of notation)
\begin{align*}
G(x)=i \qquad &\Leftrightarrow \qquad x \in [d_{i-1},d_i)
\intertext{where $d_i:= \logit^{-1}(c_i)$. Hence for $\beta \in \reell$ it holds}
\widehat{G}(x) := G(\beta x)=j \qquad &\Leftrightarrow \qquad \beta x \in [d_{i-1},d_i).
\end{align*}   
Since we will consider only values $\beta>0$ in section ... we then have
\begin{align*}
\widehat{n}^1_{ij}&=\widehat{n}^1_{ij}(\beta)= |\{\widehat{G}(x_l) =j | G(x_l)=i,\quad l=1,\ldots,N \}|\\
&= |\{1 \le l \le N	|x_l \in [d_{i-1},d_i)\cap	[d_{j-1}/\beta,d_j/\beta)	\}|.
\end{align*}   
\subsubsection{A dispersion model}
The other scenario we consider is the model $\widehat{N}^2=\widehat{N}^2(h)$ with dispersion parameter $h \ge 0$ where
\begin{align}
\widehat{n}^2_{ij}&=\widehat{n}^2_{ij}(h)= [n_i \cdot w_{ij}(h)]
\intertext{where $[\cdot]$ denotes rounding and the wheights are defined by}
w_{ij}(h) &= \frac{W_h(|i-j|)}{\sum_{l=1}^K W_h(|i-l|)}
\intertext{and $W_h$ is the kernel function(?) defined via the gauss function}
W_h(x) &=\varphi(x/h).
\end{align} 
This means that the matrix $W_h$ converges for $h \rightarrow 0$ against the identity matrix, the respective $\widehat{N}^2$ representing the ideal classifier, and in the worst case, for $h \rightarrow \infty$, the number of true borrowers per rating class is dispersed (roughly) uniformly over all rating classes. As in the case of $\widehat{N}^1$, this model is only intended as a simple way of otaining a certain kind of misclassification. 

